MAR: A structure-based search engine for models

The availability of shared software models provides opportunities for reusing, adapting and learning from them. Public models are typically stored in a variety of locations, including model repositories, regular source code repositories, web pages, etc. To profit from them developers need effective search mechanisms to locate the models relevant for their tasks. However, to date, there has been little success in creating a generic and efficient search engine specially tailored to the modelling domain. In this paper we present MAR, a search engine for models. MAR is generic in the sense that it can index any type of model if its meta-model is known. MAR uses a query-by-example approach, that is, it uses example models as queries. The search takes the model structure into account using the notion of bag of paths, which encodes the structure of a model using paths between model elements and is a representation amenable for indexing. MAR is built over HBase using a specific design to deal with large repositories. Our benchmarks show that the engine is efficient and has fast response times in most cases. We have also evaluated the precision of the search engine by creating model mutants which simulate user queries. A REST API is available to perform queries and an Eclipse plug-in allows end users to connect to the search engine from model editors. We have currently indexed more than 50.000 models of different kinds, including Ecore meta-models, BPMN diagrams and UML models. MAR is available at http://mar-search.org.

==> 031_retrieval.tex <==


Currently, there exists many kinds of text retrieval models. However, they can be summarized in these types:
%%put references
\begin{itemize}
    \item Similarity-based model. It searches the most similar documents to a query (we will consider that a query is a sequence of keywords). In general, it tries to map the query and the documents to a vector space in order to use distance metrics to measure the similarity between them.
    
    \item Probabilistic retrieval models. Using probabilistic methods, they try to estimate if a document is relevant to a given query.
    
    \item Probabilistic inference. 
    
    \item Axiomatic approach.
    
\end{itemize}

Generally speaking, our documents and queries are models. In addition, we are going to apply similarity-based approach to model retrieval. Due to that, we have to define a process that takes a model as an input and extract words or \textit{tokens}. Once we have a model as a multi-set of words, we will be able to map it to a vector space and use similarity measures.
